Quantum Critical Paraelectrics and the Casimir Effect in Time

We study the quantum paraelectric-ferroelectric transition near a quantum critical point, emphasizing the role of temperature as a "finite size effect" in time. The influence of temperature near quantum criticality may thus be likened to a temporal Casimir effect. The resulting finite-size scaling approach yields $\frac{1}{T^2}$ behavior of the paraelectric susceptibility ($\chi$) and the scaling form $\chi(\omega,T) = \frac{1}{\omega^2} F(\frac{\omega}{T})$, recovering results previously found by more technical methods. We use a Gaussian theory to illustrate how these temperature-dependences emerge from a microscopic approach; we characterize the classical-quantum crossover in $\chi$, and the resulting phase diagram is presented. We also show that coupling to an acoustic phonon at low temperatures ($T$) is relevant and influences the transition line, possibly resulting in a reentrant quantum ferroelectric phase. Observable consequences of our approach for measurements on specific paraelectric materials at low temperatures are discussed.

==> figs/qtable.tex <==
\centerline{\bf Table II. Observables for a Quantum Paraelectric with 
$D = 4$}
%
\begin{center}
\label{qscalingtab}
\begin{tabular}{|l||c|c|}
\hline
Observable & T-Dependences& g-Dependences
\\
& (g=0) & (T=0)\\
\hline
Specific Heat &  $c_v \sim T^3$
& $c_v \sim g^0$
\\
\hline
Polarization& 
$P \sim T^1$
&
$P \sim g^{\frac{1}{2}}$
\\
\hline
Susceptibility& 
$\chi \sim T^{-2}$&
$\chi \sim g^{-1}$
\\
\hline
\end{tabular}
\end{center}
%
\begin{center}
\begin{tabular}{|c|}
\hline
$P \sim E^{\frac{1}{3}}$\\
$\chi (\omega,T) = \frac{1}{\omega^2} F \left(\frac{\omega}{T} 
\right)$\\
\hline
\end{tabular}
\end{center}








